GLB: Lifeline-based Global Load Balancing library in X10

We present GLB, a programming model and an associated implementation that can handle a wide range of irregular paral- lel programming problems running over large-scale distributed systems. GLB is applicable both to problems that are easily load-balanced via static scheduling and to problems that are hard to statically load balance. GLB hides the intricate syn- chronizations (e.g., inter-node communication, initialization and startup, load balancing, termination and result collection) from the users. GLB internally uses a version of the lifeline graph based work-stealing algorithm proposed by Saraswat et al. Users of GLB are simply required to write several pieces of sequential code that comply with the GLB interface. GLB then schedules and orchestrates the parallel execution of the code correctly and efficiently at scale. We have applied GLB to two representative benchmarks: Betweenness Centrality (BC) and Unbalanced Tree Search (UTS). Among them, BC can be statically load-balanced whereas UTS cannot. In either case, GLB scales well-- achieving nearly linear speedup on different computer architectures (Power, Blue Gene/Q, and K) -- up to 16K cores.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh latex
BIBTEX=bibtex
FIG2DEV=fig2dev

NAME=glbx10
BIBNAME=x10

all: $(NAME).pdf

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)
TEX=$(NAME).tex \
    $(BIBNAME).bib \

$(NAME).dvi: $(TEX) $(EPS) $(BIBNAME).bbl
	@echo Compiling $(NAME)
	@$(LATEX) $(NAME)
	@$(MAKE) fixlabels

$(NAME).pdf: $(NAME).dvi
	@dvipdfmx -p letter $(NAME).dvi

$(NAME).ps: $(NAME).dvi
	@dvips $(NAME).dvi
	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(NAME).log),0)
	@echo $(NAME) Compiling again to fix labels
	@$(LATEX) $(NAME)
else
	@echo $(NAME) Labels are correct
endif

$(BIBNAME).bbl: $(BIBNAME).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(NAME)
	@echo Generating bibliography
	@$(BIBTEX) $(NAME)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(NAME)
	@$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(NAME).ps $(NAME).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf *.toc *.out *.bak


==> bc_orig.tex <==
% BC

\subsubsection{Problem description}
The Betweenness Centrality benchmark is taken from the SSCA2 (Scalable
Synthetic Compact Application 2) v2.2 benchmark \cite{SSCA2};
specifically, we implement the ``fourth'' kernel in this benchmark,
the computation of {\em betweenness centrality}:

\begin{quotation}
The intent of this kernel is to identify the set of vertices in the
graph with the highest betweenness centrality score. Betweenness
Centrality is a shortest paths enumeration-based centrality
metric, introduced by Freeman (1977). This is done using a betweenness
centrality algorithm that computes this metric for every vertex in the
graph. Let $\sigma_{st}$ denote the number of shortest paths between
vertices $s$ and $t$, and $\sigma_{st}(v)$ the number of those paths
passing through $v$. Betweenness Centrality of a vertex $v$ is defined
as $BC(v) = \Sigma_{s\not=v\not=t \in V} \sigma_{st}(v)/\sigma_{st}$.

The output of this kernel is a betweenness centrality score for each
vertex in the graph and the set of vertices the highest betweenness
centrality score.
\end{quotation}

We implement the Brandes' algorithm described in the benchmark,
augmenting Dijkstra's single-source shortest paths (SSSP) algorithm,
for unweighted graphs. We have implemented the exact variant of the benchmark
(\code{K4approx=SCALE}). 

The solution we implement makes one very strong assumption: that the
graph is ``small'' enough to fit in the memory of a single
place. Since the graph itself is not modified during the execution of
this benchmark, it thus becomes possible to implement this benchmark
by replicating the graph across all places. Now effectively the
computation can be performed in an embarrassingly parallel fashion. The
set of $N$ vertices is statically partitioned among $P$ places; each place is
responsible for performing the computation for the {\em source}
vertices assigned to it (for all $N$ target vertices) and computes its
local \code{betweennessMap}. After this is
done an \code{allReduce} collective performs an \code{AND} summation
    across all local \code{betweennessMaps}. 

Clearly, statically partitioning the work amongst all places in this
way is not ideal. The amount of work associated with one source node
$v$ vs another $w$ could be dramatically different. Consider for
instance a degenerate case: a graph of $N$ vertices, labeled $1\ldots
N$, with an edge $(i,j)$ if $i < j$. Clearly the work associated with
vertex $1$ is much more than the work associated with vertex $N$. 

Section~\ref{sec:bcg} discusses how to dynamically load-balance these
tasks across all places using the GLB framework (Section~\ref{sec:glb}). 

\subsubsection{Structure of the code}
The multi-place structure of this code is quite straightforward. We
use the standard at-scale X10 idiom for SPMD code:
\begin{enumerate}
\item Create a distributed data structure, accessed through a
  \code{PlaceLocalHandle} which points to an instance of a ``host''
  object (an instance of \code{SSCA2}) at each node. (Invocation of
  \code{makeFlat}.) 
\item Run the actual computation (invocation of \code{broadcastFlat}
  with the closure specifying the work to be done at each place.

  The work done in each place is the computation of a
  \code{bfsShortestPaths} for a slice of vertices from
  \code{startVertex} to \code{endVertex}. This loops through the
  vertices in the given range, computing the betweennessMap
  locally. 

  Note this computation is single threaded. It is not difficult to
  make this multi-threaded. 

\item Once the local computation has been done, and the local
  contribution to the betweennessMap computed, a
  \code{Team.WORLD.allreduce} ensures that the results are reduced and
  made available at place $0$. 
\end{enumerate}

%% \subsection{Validation.}
%% The benchmark calls for validating the algorithms by running it on a
%% graph (a torus)  with known analytical results for the betweenness
%% centrality.  Because of lack of time, we have not been able to do
%% this. If our submission is selected for presentation, we plan to
%% validate the algorithm by the time of the presentation.


%% \subsection{Performance measurement.}
%% We discuss the performance together with BC-G in Section~\ref{sec:bcg}.



==> bcg.tex <==
% BC-G

BC-G implements dynamic load-balancing by using the GLB library. Note
that this is a new capability (over what is supported by BC) -- therefore it is not surprising that
new code needs to be written and the line count is actually higher
than for BC. Specifically, \code{BCTaskFrame} and \code{BCTaskBag}
needs to be implemented, together with the invocation of the
\code{GLB} framework. A task captures a (start, end) range of
vertices. The code for \code{BCTaskFrame} is
straightforward -- it pops tasks from the \code{BCTaskBag} and for
each task executes it by calling \code{bfsShortestPaths} already
implemented in BC. The reducer takes two betweenness maps (vectors) and sums
them up pointwise.

We now consider the implementation of \code{BCTaskBag}. Our current
implementation (reported in this submission) is preliminary and in
need of further work. It is designed to satisfy the following
properties. It should be possible to find the ``mid point'' fast so
that the bag can be split in two quickly. The cost of a merge should
be low. 

The current implementation uses an array, a head pointer and a tail
pointer. The head pointer is moved forward whenever the task frame
retrieves an item and works on it. The tail pointer is used during
splitting, so it can move to the split point, copy the latter half of
the data and send it out. 

When merging, we create a new array and copy the local taskbag and the
incoming taskbag to the new array and set up the head and tail pointer
properly. We believe this copy is expensive and should be eliminated.

We believe a more careful design for this data-structure will improve
performance. Basically we need to design a data-structure that
represents a set of intervals such that two such sets can be combined
quickly and split quickly, where the split ensures that the sum of the
sizes of intervals in each half are roughly equal.  We believe that
improving the design of this data-structure will significantly improve
performance. {\em We expect to work on this in the next few
  weeks, before SuperComputing.}

\subsection{Peformance measurement}

Section~\ref{sec:bc} presents the background for the Betweenness
Centrality benchmark. There it was pointed out that the static
partitioning of the work across the given number of places may not be
ideal.  

As described in the benchmark, the application metric traversed edges
per second (TEPS) is measured as:

$$ TEPS = (8\times N \times N)/t$$

\noindent where $N$ is the number of vertices.

We now discuss results. 
All tests were run with particular parameters $(1=0.8, b=c=0.05,
d=0.1)$. This gives rise to a significantly unbalanced graph.

For Power~775 we had access to a small number of cores, and the machine was
in heavy demand, so we were unable to run long jobs.  So we chose to
vary $n$ (the log of the number of vertices) as we varied $p$. The
data is presented in a table form in Table~\ref{table:perf:bc-p7ih} to
show that $n$ varies as $P$ varies. The data shows that at these
scales, and on this architecture BC-G is quite effective in reducing
the runtime (for a given $P$ and $n$), e.g. achieving a $2x$ speed-up
for BC-G over BC.

For Blue Gene/Q and K, we show charts for a fixed $n=19$ 
(Figure~\ref{fig:perf:bc-bgq} and Figure~\ref{fig:perf:bc-k}). 
 For Blue
Gene/Q the data shows that BC-G is able to achieve around a 2x speedup
for most values of $P$. For $P=2048$, however, the performance is
somewhat comparable. For K, BC-G is generally better than BC, but with
a smaller constant. 

We believe that the representation of \code{BCTaskBag} can be
improved. The \code{split} and \code{merge} operations are expensive
and this may account for why the speedup worsens with larger $P$
because there is more contention and stealing.  {\em We expect to work
  on improving these numbers for the presentation at SC, if selected.}


\begin{figure}
\centering

$$
\begin{array}{|l|l|l|l|}
\hline
\mbox{P}&\mbox{n}&\mbox{BC (s)}&\mbox{BC-G (s)}\\ \hline \hline
1 & 16 & 78 & 109 \\ \hline
2 & 16 & 32 & 34  \\ \hline
4 & 16 & 21 & 17 \\ \hline
8 & 16 & 13 & 9 \\ \hline
16 & 17 & 35 & 19 \\ \hline
32 & 17 & 21 & 11 \\ \hline 
64 & 18 & 67 & 34 \\ \hline 
128 & 18 & 41 & 20 \\ \hline 
256 & 19 & 70 & 55 \\ \hline
\end{array}
$$
\caption{X10 Performance for BC (on Power~775)}
\label{table:perf:bc-p7ih}

\includegraphics[width=3.25in]{figures/bgq/bc-bgq.eps}
\caption{X10 Performance for BC (on Blue~Gene/Q)}
\label{fig:perf:bc-bgq}

\includegraphics[width=3.25in]{figures/k/bc-k.eps}
\caption{X10 Performance for BC (on K)}
\label{fig:perf:bc-k}
\end{figure}






==> fib.tex <==
\begin{figure}
  \centering
   \mbox{\lstinputlisting[numbers=left, mathescape,basicstyle=\ttfamily\tiny, firstline=1, lastline=100]{./ppaa2014_figures/fib.java}}
   \caption{GLB-Fibonacci example}
  \label{fig:design:fib}
\end{figure}


==> fib_old.tex <==
The code in Figure~\ref{table:fib} illustrates the use of this
framework with a simple Fibonacci computation. 

%% Add Fibonacci code in totality.

\begin{table}
{\footnotesize
\begin{verbatim}
public class FibG(n:Long) {
	static def fib(n:Long):Long=n<2? n: fib(n-1)+fib(n-2);
	
	class FibTQ implements TaskQueue{
		val bag = new ArrayListTaskBag[Long]();
		var result:Long=0;
		public def getTaskBag()=bag;
		public def getResult()= result;
		public def init(n:Long) {
			bag.bag().add(n);
		}
		public def process(var n:Long):Boolean {
			val b = bag.bag();
			for (var i:Long=0; bag.size() > 0 && i < n; i++) {
				val x = b.removeLast(); // constant time
				if (x < 2) result += x;
				else {
					b.add(x-1); // constant time
					b.add(x-2);
				}
			}
			return b.size()>0;
			
		}
		
	
		
		public def count() {
		
			return 0L;
		}
		
		public def merge(var _tb:glb.TaskBag):void {
			this.bag.merge(_tb as ArrayListTaskBag[Long]);
		}
		
	
		public def split():glb.TaskBag {
			return this.bag.split();
		}
		
		public def reduce():void {
			result= Team.WORLD.allreduce(result,Team.ADD); 
		}
		
		
	}
	//var finalResult:Long;
	public def run(n:Long):Long {
		
		val init = ()=>{ return new FibTQ(); };
		val glb = new GLB[FibTQ](init, GLBParameters.Default, true);
		
		Console.OUT.println("Starting...");
		var time:Long = System.nanoTime();
		val start = ()=>{ (glb.taskQueue()).init(n); };
		glb.run(start);
	
		 PlaceGroup.WORLD.broadcastFlat(()=>{
			(glb.taskQueue()).reduce();
		  
		});
		
		time = System.nanoTime() - time;
		Console.OUT.println("Finished.");
		Console.OUT.println("finalResult:" + glb.taskQueue().result);
		return glb.taskQueue().result;

	}
	public static def main(args:Rail[String]) {
		val N = args.size < 1 ? 10 : Long.parseLong(args(0));
		val result = new FibG(N).run(N);
		Console.OUT.println("fib(" + N + ")" + fib(N));
		Console.OUT.println("fib-glb(" + N + ")" + result);
		
	}
}
\end{verbatim}}
\caption{Fibonacci, with GLB}\label{table:fib}
\end{table}


==> glb.tex <==
% GLB
% Here we describe the basic API. This is now quite simple. user has
% to write a TaskFrame, and optionally a TaskBag, supply some
% parameters, and run the darn thing. We illustrate in running text 
% with a Fib example.

\subsection{The GLB Framework Design}
The GLB (Global Load-Balancing) framework is applicable for {\em
  tree-structured problems}. 

Such problems can be characterized thus. There is an initial
bag (multiset) of {\em tasks} (may be of size one). A task usually has a
small amount of associated state, but is permitted to access
(immutable) ``reference state''  that can be replicated across all
places. Consequently, tasks are {\em relocatable}: they can be
executed at any place. 

Tasks can be executed. Executing a task may only involve local,
self-contained work (no communication). During execution, a task is
permitted to create zero or more tasks, and produce a result of a given
(pre-specified) type \code{Z}. The user is required to specify a
reduction operator of type \code{Z}. 

The GLB framework is responsible for distributing the generated
collection of tasks across all nodes. Once no more tasks are left to
be executed, the single value of type \code{Z} (obtained by reducing
the results produced by all tasks) is returned.  

Since the execution of each task depends only on the state of the
task (and on immutable external state), the set of results produced on
execution will be the same from one run to another, regardless of
how the tasks are distributed across places. Since the user supplied
reduction operator is assumed to be associative and commutative, the
result of execution of the problem is determinate. Thus GLB is a
determinate application library that requires the user to provide a
few sequential pieces of code and handles concurrency, distribution
and communication automatically. 

The GLB framework is applicable to a wide variety of tasks. For a
simple example, consider the problem of computing the $n$'th Fibonacci
number in the naive recursive way. Here the state of the task can be
summarized by just one number (long), i.e.{} $n$. Execution of the
task yields either a result (for $n < 2$), or two tasks (for $n-1$ and
$n-2$). The results from all tasks need to be reduced through
arithmetic addition. 

All {\em state space search algorithms} from AI fall in this
category. Such algorithms are characterized by a space of states, an
initial state, and a generator function which given a state generates
zero or more states. The task is to enumerate all states (perhaps with
a cutoff), apply some function, and combine the results. An example of
such an application is the famous $N$-Queens problem.

Another example of this problem is the Unbalanced Tree Search (UTS)
benchmark. Indeed, it was our attempt to solve the UTS problem that
led to the creation of the GLB framework.

\subsection{The GLB API}
The GLB framework works by distributing bags of tasks from busy places
to idle places automatically. In special cases, the application
programmer may improve overall performance by specifying a custom
implementation of \code{TaskBag}. The implementation must support a
\code{split} operation which permits the current task bag to be split
into two (so the other piece can be distributed to another place) and
a \code{merge} operation which permits incoming work to be included in
the task bag at the current place. 

Thus in summary, the application programmer provides the following
pieces of code:
\begin{enumerate}
\item A \code{TaskFrame[Z]} class. This class is expected to maintain a
  reference to a \code{TaskBag} (the {\em local task bag}). The user
  must supply implementations for the following methods:
  \begin{enumerate}
  \item   \code{getTaskBag():TaskBag}: should return the local task bag.
  \item \code{getReducer():Reducible[Z]}: should return the reducer
    associated with this job.
  \item \code{getResult():Z}: This returns the accumulated result for all
    tasks that were completed at this place. 
  \item \code{initTask():void}: This is called once, when this task
    frame is set up at the current place. It should initialize the
    local task bag appropriately. 

    If the problem has a single root task, then the user should choose
    one place (e.g. place zero) as the place at which to add this
    task. If the problem has many initial tasks then more than one
    place may start out with non-empty task bags. 
  \item \code{runAtMostNTasks(n:Long):Boolean}: This method must run at most
    \code{n} tasks from the task bag at the current place, and return
    \code{true} if there is still work left to do in the local task
    bag. During the execution of this method, user code may manipulate
    the local task bag freely (removing and adding tasks to it). The
    framework guarantees that no other worker will concurrently access
    the task bag. For tasks which have completed and produced a result
    of type \code{Z}, the method must accumulate the result in local
    state, using the supplied reducer.
\end{enumerate}
\item Optionally, a custom class extending \code{TaskBag} and
  appropriately implementing \code{split} and \code{merge} methods. 
\end{enumerate}

The framework is invoked in a fairly simple way:

{\footnotesize
\begin{verbatim}
val r = new GlobalLoadBalancer[T](parameters);
val result = g.run(()=> new TaskFrameImp[T]());
\end{verbatim}}

\noindent First an instance of \code{GlobalLoadBalancer} is created
with a specification of parameters for controlling various aspects of
global load-balancing. Next the framework is invoked, supplying a
function that generates an instance of the user-specified
\code{TaskFrame} class, with the appropriate result type. This method
returns the result of running the user's problem, balanced across all
places. 

The code in Figure~\ref{table:fib} illustrates the use of this
framework with a simple Fibonacci computation. 

%% Add Fibonacci code in totality.

\begin{table}
{\footnotesize
\begin{verbatim}
package fib;

import glb.TaskBag;
import glb.TaskFrame;
import glb.GlobalLoadBalancer;
import glb.ArrayListTaskBag;
import glb.GLBParameters;

public class Fib(n:Long) {
    class FibFrame extends TaskFrame[Long] {
        val bag = new ArrayListTaskBag[Long]();
        val reducer = Reducible.SumReducer[Long]();
        var result:Long=0;
        public def getTaskBag()=bag;
        public def getReducer()=reducer;
        public def getResult()= result;
        public def initTask() {
            if (here.id==0) bag.bag().add(n);
        }
        public def runAtMostNTasks(n:Long) {
            val b = bag.bag();
            for (1..n) {
                if (b.size()<=0) break;
                val x = b.removeLast(); // constant time
                if (x < 2) result += x;
                else {
                    b.add(x-1); // constant time
                    b.add(x-2);
                }
            }
            return b.size()>0;
        }
    }
    public def run():Long {
        val g = new GlobalLoadBalancer[Long](GLBParameters.Default);
        return g.run(()=>new FibFrame());
    }
    static def fib(n:Long):Long=n<2? n: fib(n-1)+fib(n-2);
    public static def main(args:Rail[String]) {
        val N = args.size < 1 ? 10 : Long.parseLong(args(0));
        val result = new Fib(N).run();
        
        Console.OUT.println("fib(" + N + ")=" 
           + result + " (actual=" + fib(N)+")");
    }
}
\end{verbatim}}
\caption{Fibonacci, with GLB}\label{table:fib}
\end{table}

\subsection{Implementation}

GLB is essentially a library form of UTS. Hence the basic structure of
the code is the same as for UTS. 


\subsection{Validation}
We have implemented three benchmarks using this framework --
Fibonacci, UTS and BC. In each case, for various input sizes we
checked the result obtained for these benchmarks with results obtained
through alternative means (e.g. running the benchmarks directly), and
verified the results were the same.

\subsection{Performance} Performance is reported in the UTS-G
and BC-G sections, through the performance of those benchmarks
compared with UTS and BC, respectively.


==> uts_orig.tex <==

\subsubsection{UTS description}
The Unbalanced Tree Search benchmark measures the rate of traversal of
a tree generated on the fly using a splittable random number
generator. For this submission, we used a \emph{fixed geometric law}
for the random number generator with branching factor $b_0=4$, seed
$r=19$, and tree depth $d$ varying from 13 to 20 depending on core counts and architecture.

\begin{quote}
The nodes in a geometric tree have a branching factor that follows a
geometric distribution with an expected value that is specified by the  
parameter $b_0 > 1$. The parameter $d$ specifies its maximum depth
cut-off, beyond which the tree is not allowed to grow ... The expected
size of these trees is $(b_0)^d$, but since the geometric distribution
has a long tail, some nodes will have significantly more than $b_0$
children, yielding unbalanced trees. 
\end{quote}

The depth cut-off makes it possible to estimate the size of the trees
and shoot for a target execution time. To be fair, the distance from
the root to a particular node is never used in our benchmark
implementation to predict the size of a subtree. In other words, all
nodes are treated equally, irrespective of the current depth.  

\subsubsection{Design}

The material in this section is excerpted from \cite{glb}, and
unchanged from our 2012 HPCC submission.

One common way to load balance is to use {\em work-stealing}. For
shared memory system this technique has been pioneered in the Cilk
system.  Each worker maintains a double ended queue (deque) of tasks. When a
worker encounters a new task, it pushes its continuation onto the
bottom of the deque, and descends into the task. On completion of the task, it
checks to see if its deque has any work, if so it pops a task (from the
bottom) and continues with the work. Else (its deque is empty) it
looks for work on other workers' deques. It randomly determines a {\em
  victim} worker, checks if its queue is non-empty, and if so, pops a
task from the top of the deque (the end other than the one being
operated on by the owner of the deque).  If the queue is empty, it
guesses again and continues until it finds work. Work-stealing systems
are optimized for the case in which the number of steals is much
smaller than the total amount of work. This is called the ``work
first'' principle -- the work of performing a steal is incurred by the
thief (which has no work), and not the victim (which is busy
performing its work). 

Distributed work-stealing must deal with some additional
complications. First, the cost of stealing is usually significantly
higher than in the shared memory case. For many systems, the target
CPU must be involved in processing a steal attempt. Additionally, one
must solve the distributed termination detection problem. The system
must detect when all workers have finished their work, and there is no
more work. At this point all workers should be shut down, and the
computation should terminate. 

X10 already offers a mechanism for distributed termination detection
-- \texttt{finish}. Thus, in principle it should be possible to spawn
an activity at each place, and let each look for work. To trigger
\texttt{finish} based termination detection however, these workers
must eventually terminate. But when? One simple idea is that a worker
should terminate after $k$ steal attempts have failed. However this
leaves open the possibility that a worker may terminate too early --
just because it happened to be unlucky in its first $k$ guesses. If
there is work somewhere else in the network then this work
can no longer be shared with these terminated workers, thereby
affecting parallel efficiency. (In an extreme case this could lead to
sequentialize significant portion of the work.) 

Therefore there must be a way by which a new activity can be launched 
at a place whose worker has already terminated. This leads to the idea
of a {\em lifeline graph}. For each place $p$ we pre-determine a set of
other places, called {\em buddies}. Once the worker at $p$ has
performed $k$ successive (unsuccessful) steals, it examines its
buddies in turn. At each buddy it determines whether there is some
work, and if so, steals a portion. However, if there is no work, it
records at the buddy that $p$ is waiting for work. If $p$ cannot find
any work after it has examined all its buddies, it dies -- the place $p$
now becomes quiescent.  

But if $P$ went to a buddy $B$, and $B$ did not have any work, then
it must itself be out looking for work -- hence it is possible that it
will soon acquire work. In this case we require that $B$ {\em
  distribute} a portion of the work to those workers that attempted to
buddy steal from it but failed. Work must be spawned on its own
\texttt{async} -- using the \texttt{at (p) async S} idiom. If $P$ had
 no activity left, it now will have a fresh activity. Thus, unlike
 pure work-stealing based systems, a system with lifeline graphs will
 see its nodes moving from a state of processing work (the active state), to a state in
 which they are stealing to a state in which they are dead, to a state
 (optionally) in which they are woken up again with more work (and are
 hence back in the active state).  

Note that when there is no work in the system, all places will be dead,
there will be no active \texttt{async} in the system and hence the
top-level \texttt{finish} can terminate. 

The only question left is to determine the assignment of buddies to a
place. We are looking for a directed graph that is fully connected (so
work can flow from any vertex to any other vertex) and that has a low
diameter (so latency for work distribution is low) and has a low
degree (so the number of buddies potentially sending work to a dead
vertex is low).  $z$-dimensional hyper-cubes  satisfy these properties
and have been implemented. 

\subsubsection{Implementation}\label{sec:uts-inline}
Our implementation follows from \cite{glb} and includes the
performance improvements described in our HPCC 2012 submission
(using \code{FINISH\_DENSE} to reduce the overhead of termination
detection), using \code{@Uncounted} asyncs,  and using a compact
representation of the active nodes in a place using an implicit (lower,
upper) bounds representation rather than an explicit enumeration.

We have made a change in how the native SHA1 code is integrated into
X10. Consequently we replaced all of the 169 lines of very complex C++ wrapper code
with 3 native annotations (i.e., 3 lines of C code embedded into X10) as for instance in:

{\small
\begin{verbatim}
def this(seed:Int, depth:Int) {
  @Native("c++", "rng_init((RNG_state*)this, seed);") {}
  this.depth = depth;
}
\end{verbatim}
}

We fixed a nasty deadlock condition when using multi-dimensional lifeline graphs.


\subsubsection{Verification}
The code was validated by checking the results for specific
configurations against pre-computed numbers. 


% Runs on MPI now ... were there any issues here?
\subsubsection{UTS-GLB}\label{sec:utsg}
UTS-G is a variant of UTS written using the GLB library. The code for
\code{GlobalLoadBalancer} and \code{LocalJobRunner} is no longer
needed, since they are part of the library. The code for managing bags
of tasks is refactored into a \code{UTSTaskBag} class. Similarly the
code for executing a UTS task \code{runATMostNTasks} in
\code{UTSTaskFrame} is similarly very straightforward.  The native
code (for SHA1 hashes) remains unchanged -- it belongs in the
application and not the library.

Thanks to the GLB library the number of X10 LOCs drops from 493 for UTS to 225 for UTS-G.

%% \subsection{Performance}
%% \begin{figure}
%% \centering
%% \includegraphics[width=3.25in]{figures/p7ih/uts-p7ih.eps}
%% \caption{X10 Performance for UTS (on Power~775)}
%% \label{fig:perf:uts-p7ih}

%% \includegraphics[width=3.25in]{figures/bgq/uts-bgq.eps}
%% \caption{X10 Performance for UTS (on Blue~Gene/Q)}
%% \label{fig:perf:uts-bgq}

%% \includegraphics[width=3.25in]{figures/k/uts-k.eps}
%% \caption{X10 Performance for UTS (on K)}
%% \label{fig:perf:uts-k}
%% \end{figure}

%% We report performance for UTS and UTS-G.

%% On Power~775, as we demonstrated in our 2012 HPCC Submission, UTS achieves linear speedup up to 50,000 cores. UTS-G is only marginally slower.

%% On Blue~Gene/Q and K however, we ran the code ``as is'' without having the time to tune the main parameters of the load balancer to the specifics of the architecture. These parameters include the mapping of the lifeline graph onto the network axes (especially the dimensionality) as well as the frequency of network probes. With proper tuning, we believe we can redress the curves dramatically. In essence, with our implementation and our 2012 runs at scale on Power~775, we established that the benchmark (for this family of trees at least) is compute bound.

%% On Blue~Gene/Q, the sequential performance of the UTS-G code is 15\% less than the UTS code: the higher-order implementation confuses the optimizer of the backend compiler (xlC). This is not the case on other platforms. As a result, UTS-G appears to scale better than UTS, but this is misleading.
%% At scale, they are more or less on par as UTS only achieves 60\% efficiency for now. Hence the sequential inefficiency of UTS-G can hide behind the latency of the load balancer.

%% The measurements on K are very preliminary. The code runs and computes correct results. The performance is under investigation.



%We discuss the performance together with UTS-G in Section~\ref{sec:utsg}.
%\todo{Performance analysis. Why are numbers bad for the K. Is
%  there some basic operation that is slow on the K?}

